IntRepair: Informed Repairing of Integer Overflows

Integer overflows have threatened software applications for decades. Thus, in this paper, we propose a novel technique to provide automatic repairs of integer overflows in C source code. Our technique, based on static symbolic execution, fuses detection, repair generation and validation. This technique is implemented in a prototype named IntRepair. We applied IntRepair to 2,052C programs (approx. 1 million lines of code) contained in SAMATE's Juliet test suite and 50 synthesized programs that range up to 20KLOC. Our experimental results show that IntRepair is able to effectively detect integer overflows and successfully repair them, while only increasing the source code (LOC) and binary (Kb) size by around 1%, respectively. Further, we present the results of a user study with 30 participants which shows that IntRepair repairs are more than 10x efficient as compared to manually generated code repairs

==> IntRepair_ TSE19 Journal/old-text.tex <==
%% OLD TEXT from Background about Codan


% Codan contains a component for static detection of integer overflow. During symbolic execution, when an assignment statement is encountered, the {\textit{integer overflow detection}} component is asked to check if there is an integer overflow error or not.

%%was removed since it is boring 
% In brief, the Codan engine has the following main features:
% (1) unrestricted context depth,
% (2) program loop unrolling customizations (\textit{i.e.,} currently each loop is unrolled \textit{k} times),
% (3) external library calls are supported through stub functions,
% (4) search for more relevant program paths,
% (5) automatic slicing of SMT equation systems,
% (6) logic representation based on uninterpreted functions and non-linear integer and real arithmetic (AUFNIRA),
% (7) program path validation, 
% (8) SMT solving based on the Z3 SMT solver,
% (9) path-sensitive tracing of shared variables, 
% (10) support for translation of deep nested \verb!C! structs into SMT logic, and
% (11) Eclipse IDE plug-in support.

% Note that our symbolic execution engine has the following main features:
% \begin{enumerate}
% \item\textbf{Unrestricted Context Depth.}
% Our symbolic execution engine performs an inter-procedural path-sensitive 
% analysis with a call string approach~\cite{khedker:flow, sharir:pnueli}.
% For each function a CFG is built. The function call context is represented by a program path leading to its call. 
% 
% \item\textbf{Loop Unrolling Trade-offs.}
% Each program loop can be unrolled up to a certain depth or set to be unlimited. Currently, we unroll each loop up to 10 times.
% We are aware that this might incur accuracy degradation and make our approach to be unsound since not all 
% possible program paths can be analyzed. It is also possible to leave loop unrolling unconstrained, which 
% can lead in some cases to non-termination (\textit{e.g.,} endless loops) where the number of loop iterations is not known upfront.
% 
% \item\textbf{Library Calls.}
% Library calls, such as  \texttt{memset} and \texttt{memcpy}, can be handled by providing a stub function for each of these functions in advance,
% which can model their behavior: 1) required (consumed) variables, 2) returned variables, 
% 3) side effects on parameters.
% %3) operations performed on the variables of each of these functions, and 
% %4) SMT constraints which model interaction of the variables used as parameters for these functions with other variables that are attached to the corresponding symbolic variables. 
% 
% During the static program analysis, when a library function is encountered, one of the available library modeling functions is used by the engine interpreter.
% We assume that for each analyzed program containing a library function call, we have the corresponding stub function defined upfront inside our engine.
% 
% \item\textbf{Finding Program Paths.}
% We use a fixed deterministic thread scheduling algorithm for running the symbolic execution.
% The symbolic execution is run with approximate path coverage which uses \textit{depth-first search} (DFS). 
% During DFS, program states are backtracked and branch decisions are changed.
% The loop iteration bound can be configured either to prune a path until the loop 
% iteration bound is reached or to bypass the loop by avoiding the branch validation check.
% 
% \item\textbf{Automatic Slicing.}
% The goal of automatic slicing~\cite{tip1994survey} is to keep the system of satisfiability checks as small as possible.
% For this reason only relevant logic equations are passed to the solver for 
% verification. We perform automatic slicing over the data flow in order to verify conditions on a program path 
% and over the control flow to separate the analysis of different program paths.
% %\item\textbf{Context Sharing for Different Checkers.}
% %Our engine allows that multiple checkers (\textit{\textit{e.g.,}} integer overflow, buffer overflow, race condition, etc.) run in parallel
% %during symbolic execution. The checkers are allowed to share the contexts because there is separation from the 
% %symbolic path interpretation. Each checker is allowed to receive notifications from a symbolic interpreter
% %in order to query context equations.
% 
% \item\textbf{Logic Representation.}
% We use the SMT-LIB sub-logic of arrays, uninterpreted functions and non-linear integer and real
% arithmetic (AUFNIRA) since this approach can be automatically decided. Pointers for example are handled as symbolic 
% pointers by the engine interpreter with a target and a symbolic integer as offset formula
% and outputted as logical formulas when dereferenced.
% 
% \item\textbf{Path Validation.} %8
% %The path validation is triggered at branch nodes and uses the same interface as the checkers.
% %For all path decisions up to the current branch the 
% %path validator queries the equation SMT-LIB linear system slice.
% Path validator checks the satisfiability of path constraints on branch nodes in an incremental manner.
% The path validator throws a path unsatisfiable exception if the solver answer is unsatisfiable;
% then the symbolic execution proceeds with the next path.
% 
% \item\textbf{SMT Solving.} %9
% SMT solving is used for three main purposes: 1) for checking satisfiable and un-satisfiable program execution paths. This helps to assess if certain program location can be reached during 
% normal program execution. 2) for checking the presence of an integer overflow. Additional SMT constraints are
% added to SMT linear constraint system to check for the presence of an integer overflow. 3) for 
% checking if a repair removes an integer overflow. 
% Note that for solving all the SMT constraints, we use the Z3~\cite{z3} 
% solver because of its precision and reduced runtime overhead.
% 
% \item\textbf{Path-sensitive Tracing of Shared Variables.} %10
% It is possible to use shared variables between threads in a context-sensitive way. 
% This is accomplished by first marking all global shared variables, and then the shared property is inferred over 
% data flow constructs such as references, assignments, function call parameters and return values.
% 
% %\item\textbf{Posix Threads Support.} %11
% %We can accommodate environment functions by specifying symbolic models of library functions.
% %In this way, the interaction with the environment can be simulated.
% 
% \item\textbf{Deep Nested \verb!C! Structs.} %12
% %The \verb!C! language program statement to SMT translator engine component
% Our SMT translation engine
%  is designed to recursively traverse deep nested \verb!C/C++! structures
% in order to determine the real type of a field inside the struct. Accordingly, our tool does not lose precision when dealing with \verb!C! structs data types.

%\item\textbf{Eclipse Extension} %13
%Our engine is integrated into the Eclipse CDT API as a plug-in for the following main reasons:
%\textit{1)} to be able to parse \verb!C/C++! code, \textit{2)} to build a CFG
%of the code \textit{3)} to allow for precise analysis of program statements with an abstract syntax tree (AST) visitor, and 
%\textit{4)} to translate source code program statements to SMT constraints.

% \end{enumerate}













\textbf{Automated Mode.} In this mode, the static analysis is triggered after each new bug repair was inserted into
the program. In case that after an analysis run \sysname finds a bug then a new bug 
report will be filed and the programmer has the possibility to manually check in this way if the old bug was completely removed 
or a new bug was detected.

% old text from intro
We implemented our approach into a tool, \sysname which can detect and generate correct repairs by transferring SMT constraints 
from the fault location step to bug repair generation and solving these constraints with the help of the Z3 SMT solver \cite{z3}.
\sysname uses tailored \textit{symbolic execution}~\cite{klee, intscope, cadar2013symbolic, avgerinos2014enhancing, marinescu2012make} 
to provide a fused \textit{detection}, \textit{repair}, and \textit{validation} approach for \verb!C! source code programs.
Note, that our repair generation technique is general enough to be implemented on top of other symbolic execution engines as well.



==> old-text.tex <==
%% OLD TEXT from Background about Codan


% Codan contains a component for static detection of integer overflow. During symbolic execution, when an assignment statement is encountered, the {\textit{integer overflow detection}} component is asked to check if there is an integer overflow error or not.

%%was removed since it is boring 
% In brief, the Codan engine has the following main features:
% (1) unrestricted context depth,
% (2) program loop unrolling customizations (\textit{i.e.,} currently each loop is unrolled \textit{k} times),
% (3) external library calls are supported through stub functions,
% (4) search for more relevant program paths,
% (5) automatic slicing of SMT equation systems,
% (6) logic representation based on uninterpreted functions and non-linear integer and real arithmetic (AUFNIRA),
% (7) program path validation, 
% (8) SMT solving based on the Z3 SMT solver,
% (9) path-sensitive tracing of shared variables, 
% (10) support for translation of deep nested \verb!C! structs into SMT logic, and
% (11) Eclipse IDE plug-in support.

% Note that our symbolic execution engine has the following main features:
% \begin{enumerate}
% \item\textbf{Unrestricted Context Depth.}
% Our symbolic execution engine performs an inter-procedural path-sensitive 
% analysis with a call string approach~\cite{khedker:flow, sharir:pnueli}.
% For each function a CFG is built. The function call context is represented by a program path leading to its call. 
% 
% \item\textbf{Loop Unrolling Trade-offs.}
% Each program loop can be unrolled up to a certain depth or set to be unlimited. Currently, we unroll each loop up to 10 times.
% We are aware that this might incur accuracy degradation and make our approach to be unsound since not all 
% possible program paths can be analyzed. It is also possible to leave loop unrolling unconstrained, which 
% can lead in some cases to non-termination (\textit{e.g.,} endless loops) where the number of loop iterations is not known upfront.
% 
% \item\textbf{Library Calls.}
% Library calls, such as  \texttt{memset} and \texttt{memcpy}, can be handled by providing a stub function for each of these functions in advance,
% which can model their behavior: 1) required (consumed) variables, 2) returned variables, 
% 3) side effects on parameters.
% %3) operations performed on the variables of each of these functions, and 
% %4) SMT constraints which model interaction of the variables used as parameters for these functions with other variables that are attached to the corresponding symbolic variables. 
% 
% During the static program analysis, when a library function is encountered, one of the available library modeling functions is used by the engine interpreter.
% We assume that for each analyzed program containing a library function call, we have the corresponding stub function defined upfront inside our engine.
% 
% \item\textbf{Finding Program Paths.}
% We use a fixed deterministic thread scheduling algorithm for running the symbolic execution.
% The symbolic execution is run with approximate path coverage which uses \textit{depth-first search} (DFS). 
% During DFS, program states are backtracked and branch decisions are changed.
% The loop iteration bound can be configured either to prune a path until the loop 
% iteration bound is reached or to bypass the loop by avoiding the branch validation check.
% 
% \item\textbf{Automatic Slicing.}
% The goal of automatic slicing~\cite{tip1994survey} is to keep the system of satisfiability checks as small as possible.
% For this reason only relevant logic equations are passed to the solver for 
% verification. We perform automatic slicing over the data flow in order to verify conditions on a program path 
% and over the control flow to separate the analysis of different program paths.
% %\item\textbf{Context Sharing for Different Checkers.}
% %Our engine allows that multiple checkers (\textit{\textit{e.g.,}} integer overflow, buffer overflow, race condition, etc.) run in parallel
% %during symbolic execution. The checkers are allowed to share the contexts because there is separation from the 
% %symbolic path interpretation. Each checker is allowed to receive notifications from a symbolic interpreter
% %in order to query context equations.
% 
% \item\textbf{Logic Representation.}
% We use the SMT-LIB sub-logic of arrays, uninterpreted functions and non-linear integer and real
% arithmetic (AUFNIRA) since this approach can be automatically decided. Pointers for example are handled as symbolic 
% pointers by the engine interpreter with a target and a symbolic integer as offset formula
% and outputted as logical formulas when dereferenced.
% 
% \item\textbf{Path Validation.} %8
% %The path validation is triggered at branch nodes and uses the same interface as the checkers.
% %For all path decisions up to the current branch the 
% %path validator queries the equation SMT-LIB linear system slice.
% Path validator checks the satisfiability of path constraints on branch nodes in an incremental manner.
% The path validator throws a path unsatisfiable exception if the solver answer is unsatisfiable;
% then the symbolic execution proceeds with the next path.
% 
% \item\textbf{SMT Solving.} %9
% SMT solving is used for three main purposes: 1) for checking satisfiable and un-satisfiable program execution paths. This helps to assess if certain program location can be reached during 
% normal program execution. 2) for checking the presence of an integer overflow. Additional SMT constraints are
% added to SMT linear constraint system to check for the presence of an integer overflow. 3) for 
% checking if a repair removes an integer overflow. 
% Note that for solving all the SMT constraints, we use the Z3~\cite{z3} 
% solver because of its precision and reduced runtime overhead.
% 
% \item\textbf{Path-sensitive Tracing of Shared Variables.} %10
% It is possible to use shared variables between threads in a context-sensitive way. 
% This is accomplished by first marking all global shared variables, and then the shared property is inferred over 
% data flow constructs such as references, assignments, function call parameters and return values.
% 
% %\item\textbf{Posix Threads Support.} %11
% %We can accommodate environment functions by specifying symbolic models of library functions.
% %In this way, the interaction with the environment can be simulated.
% 
% \item\textbf{Deep Nested \verb!C! Structs.} %12
% %The \verb!C! language program statement to SMT translator engine component
% Our SMT translation engine
%  is designed to recursively traverse deep nested \verb!C/C++! structures
% in order to determine the real type of a field inside the struct. Accordingly, our tool does not lose precision when dealing with \verb!C! structs data types.

%\item\textbf{Eclipse Extension} %13
%Our engine is integrated into the Eclipse CDT API as a plug-in for the following main reasons:
%\textit{1)} to be able to parse \verb!C/C++! code, \textit{2)} to build a CFG
%of the code \textit{3)} to allow for precise analysis of program statements with an abstract syntax tree (AST) visitor, and 
%\textit{4)} to translate source code program statements to SMT constraints.

% \end{enumerate}













\textbf{Automated Mode.} In this mode, the static analysis is triggered after each new bug repair was inserted into
the program. In case that after an analysis run \sysname finds a bug then a new bug 
report will be filed and the programmer has the possibility to manually check in this way if the old bug was completely removed 
or a new bug was detected.

% old text from intro
We implemented our approach into a tool, \sysname which can detect and generate correct repairs by transferring SMT constraints 
from the fault location step to bug repair generation and solving these constraints with the help of the Z3 SMT solver \cite{z3}.
\sysname uses tailored \textit{symbolic execution}~\cite{klee, intscope, cadar2013symbolic, avgerinos2014enhancing, marinescu2012make} 
to provide a fused \textit{detection}, \textit{repair}, and \textit{validation} approach for \verb!C! source code programs.
Note, that our repair generation technique is general enough to be implemented on top of other symbolic execution engines as well.


